Bethe--Salpeter wave functions in integrable models

We investigate some properties of Bethe--Salpeter wave functions in integrable models. In particular we illustrate the application of the operator product expansion in determining the short distance behavior. The energy dependence of the potentials obtained from such wave functions is studied, and further we discuss the (limited) phenomenological significance of zero--energy potentials.

==> sect_wf_Ising <==
\section{Ising Model}

The S-matrix operator is given by
\be
{\bf S}=(-1)^{{\bf N}({\bf N}-1)/2}
\end{equation}
where ${\bf N}$ is the particle number operator. An energy
independent phase is not observable in a scattering experiment; 
however the non-trivial S-matrix reflects the fact
that the off shell correlation functions are not those of a free field.

Generalized form factors are given by
\ba
&&\phantom{}^{\rm out}\langle\theta_1,\dots,\theta_t|\sigma(0)|
\theta_{t+1},\dots,\theta_N\rangle^{\rm in}
\nonumber\\
&&=(2i)^{(N-1)/2}\prod_{1\le i<j\le t}T(|\theta_i-\theta_j|)
\prod_{1\le r\le t<s\le N}\frac{\cal P}{T(\theta_r-\theta_s)}
\prod_{t<k<l\le N} T(|\theta_k-\theta_l|)\,,
\nonumber\\
&&
\ea
with $N$ an odd positive integer. ${\cal P}$ denotes the principle part and
\be
T(x)\equiv\tanh\frac{x}{2}\,.
\end{equation}
The state normalization is
\be
\langle \theta|\theta'\rangle=4\pi\delta(\theta-\theta')
\end{equation}
for states with momenta $p=M(\ch\theta,\sh\theta)$ and rapidity $\theta$.
The sum over states is
\be
1=|0\rangle\langle 0|+\sum_{r=1}^\infty
\int_{-\infty}^\infty \frac{\rmd\theta_1}{4\pi}
\int_{-\infty}^{\theta_1}\frac{\rmd\theta_2}{4\pi}
\dots
\int_{-\infty}^{\theta_{r-1}}\frac{\rmd\theta_r}{4\pi}
|\theta_1,\dots,\theta_r\rangle^{\rm s}\phantom{}^{\rm s}
\langle \theta_1,\dots,\theta_r|
\end{equation}
where s stands for in or out.
It is often convenient for fixed $r$ to change variables to
\ba
u_j&=&\theta_j-\theta_{j+1},\,\,\,\,j=1,\dots,r-1\,,
\\
\Lambda&=&\frac12\ln\left(
\frac{\sum_j\rme^{ \theta_j}}
     {\sum_j\rme^{-\theta_j}}\right)\,,
\ea
since in terms of these variables the total energy and momentum take
on the simpler form:
\be
M\left(\sum_{j=1}^r\ch\theta_j,\sum_{j=1}^r\sh\theta_j\right)
=M^{(r)}({\bf u})(\ch\Lambda,\sh\Lambda)
\end{equation}
where
\be
M^{(r)}({\bf u})=M\left[r+2\sum_{1\le i<j\le r-1}
\ch(u_{ij})\right]^{1/2}\,,
\end{equation}
where we have introduced the notation
\be
u_{ij}\equiv u_i+\dots+u_j\,,\,\,\,\,i\le j\,,\,\,\,(u_{ii}=u_i)\,.
\end{equation}
Correspondingly the integration measures above are replaced by
\be
\int_{-\infty}^\infty    \frac{\rmd\theta_1}{4\pi}
\int_{-\infty}^{\theta_1}\frac{\rmd\theta_2}{4\pi}
\dots
\int_{-\infty}^{\theta_{r-1}}\frac{\rmd\theta_r}{4\pi}
\rightarrow
\int_0^\infty\frac{\rmd^{r-1} u}{(4\pi)^{r-1}}\int_{-\infty}^\infty
\frac{\rmd\Lambda}{4\pi}
\end{equation}
We also have the inverse transformation
\be
\theta_j=u_{jr}+\Lambda\,,\,\,\,\,\,j=1,\dots,r\,,
\end{equation}
with
\be
u_r\equiv\frac12\ln\left(
\frac{1+\sum_{j=1}^{r-1}\rme^{-u_{j(r-1)}}}
     {1+\sum_{j=1}^{r-1}\rme^{ u_{j(r-1)}}}\right)\,.
\end{equation}
The field is normalized by
\be
\langle 0|\sigma(x)|p\rangle=\rme^{-ipx}\,.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Vacuum 2--point functions}

Define the vacuum 2--point functions
\footnote{Note that $\sigma,\mu$ are in Fronseca and 
Zamolodchikov are interchanged with respect to ours.
Also the field normalization differs.}:
\ba
G(r)&=&\langle 0|\sigma((0,x_1))\sigma(0)|0\rangle\,,
\\
\widetilde{G}(r)&=&\langle 0|\mu((0,x_1))\mu(0)|0\rangle\,,
\ea
For the sum and difference
\be
G_\pm(r)=\widetilde{G}(r)\pm G(r)\,,
\label{Gplusminus}
\end{equation}
we have
\be
G_\pm(r)=\rme^{\chi(r)/2}\rme^{\pm\varphi(r)/2}\,,
\end{equation}
where the functions $\chi,\varphi$ obey the equations
\ba
\frac{1}{r}[r\varphi'(r)]'&=&\frac12\sh(2\varphi(r))\,,
\\
\frac{1}{r}[r\chi'(r)]'&=&\frac12[1-\ch(2\varphi(r))]\,.
\ea
Note $\varphi^{\prime2}=\chi'/r-\chi''$. In particular we have
\be
G(r)=\rme^{\chi(r)/2}\sinh\left(\frac{\varphi(r)}{2}\right)\,.
\end{equation}

The short distance behaviors of $\varphi,\chi$ are given by
\ba
\rme^{-\varphi(r)}&\sim&-\frac12 r\Omega(r)+\rmO(r^4)\,, 
\\
\rme^{\chi(r)}&\sim&-2C_\chi^2\sqrt{r}\Omega(r)+\rmO(r^2)\,, 
\ea
where
\be
\Omega(r)=\ln(kr)\,,\,\,\,\,\,\,\,k=\frac18\rme^\gamma\,,
\end{equation}
and
\be
C_\chi=2^{-7/6}A^{-3}\rme^{1/4}=0.27119012339\dots\,,
\end{equation}
where 
\be
A=\exp\left\{\frac{1}{12}-\zeta'(-1)\right\}=1.282427\dots
\end{equation} is Glaisher's constant. This implies for small $r$
\be
G(r)\sim C_\chi r^{-1/4}+\rmO(r^{1/4})\,.
\end{equation}

Next for long distances:
\ba
\varphi(r)&=&\frac{2}{\pi}K_0(r)+\rmO(\rme^{-3r})\,,
\\
\chi(r)&=&-2\ln2-\frac{2r}{\pi^2}\left[r\{K_0(r)^2-K_1(r)^2\}+
K_0(r)K_1(r)\right]+\rmO(\rme^{-4r})\,.
\ea

Note the modified Bessel function 
\ba
K_0(|r|)&=&\int_0^\infty\rmd z\,\rme^{-|r|\ch z}\,,
\\
&=&\int_0^\infty\rmd v\,\cos(|r|\sh v)\,,
\label{besselK0}
\ea
behaves for small $|r|$ as
\be
K_0(|r|)=-\ln\left(\frac{|r|}{2}\right)-\gamma+\rmO(|r|^2)\,,
\end{equation}
and for large $r$,
\ba
K_0(|r|)&=&\sqrt{\frac{\pi}{2|r|}}\rme^{-|r|}
\left[1-\frac{1}{8|r|}+\dots\right]\,,
\\
K_1(|r|)&=&\sqrt{\frac{\pi}{2|r|}}\rme^{-|r|}
\left[1+\frac{3}{8|r|}+\dots\right]\,.
\ea

\subsubsection{1-- and 3--particle approximations}

The vacuum two-point function $G(r)$
can be expressed as a sum over $s$--particle contributions:
\be
G(r)=\sum_{s=1}^{\infty}G_{2s-1}(r)\,.
\end{equation}

For the 1--particle contribution:
\ba
G_1(r)&=&\frac{1}{4\pi}\int_{-\infty}^\infty\rmd\theta_1\,\rme^{ir\sh\theta_1}
\\
&=&\frac{1}{2\pi}K_0(|r|)\,.
\ea

For the 3--particle contribution:
\ba
G_3(r)&=&\frac{1}{16\pi^3}\int_0^\infty\rmd u_1\,\rmd u_2
\int_{-\infty}^\infty \rmd\Lambda\,\rme^{i|r|\mu^{(3)}(u)\sh\Lambda}
\left[T(u_1)T(u_2)T(u_1+u_2)\right]^2
\nonumber\\
&&
\\
&=&\frac{1}{8\pi^3}\int_0^\infty\rmd u_1\,\rmd u_2
\int_0^\infty \rmd\Lambda\,\rme^{-|r|\mu^{(3)}(u)\ch\Lambda}
\left[T(u_1)T(u_2)T(u_1+u_2)\right]^2\,.
\nonumber\\
&&
\ea


\begin{table}[h]
\centering
\begin{tabular}[t]{l|l|l|l|l|l}
\hline
$r$ &
$G_1(r)$\quad\,\,\,&
$G_3(r)$\quad\,\,\,&  
$G_1(r)+G_3(r)$\quad\,\,\,&  
$G(r)$\quad\,\,\,&  
$C_\chi r^{-1/4}$\\[1.0ex]
\hline \hline
$10.0$&$2.8298\rme-6$&$1.6988\rme-21$&$2.8298\rme-6$&$2.8298\rme-6$&\\[1.0ex]
$5.0$&$5.8746\rme-4$&$8.1809\rme-14$&$5.8746\rme-4$&$5.8746\rme-4$&\\[1.0ex]
$4.0$&$1.7761\rme-3$&$3.7219\rme-12$&$1.7761\rme-3$&$1.7761\rme-3$&\\[1.0ex]
$3.0$&$5.5290\rme-3$&$2.0606\rme-10$&$5.5290\rme-3$&$5.5290\rme-3$&\\[1.0ex]
$2.0$&$1.8127\rme-2$&$1.5904\rme-8$&$1.8127\rme-2$&$1.8127\rme-2$&\\[1.0ex]
$1.0$&$6.7008\rme-2$&$2.5092\rme-6$&$6.7011\rme-2$&$6.7007\rme-2$&\\[1.0ex]
$0.1$&$3.8628\rme-1$&$4.4679\rme-3$&$3.9075\rme-1$&$3.9075\rme-1$&\\[1.0ex]
$0.01$&$7.5141\rme-1$&$7.9626\rme-2$&$8.3104\rme-1$&$8.3140\rme-1$&$8.576\rme-1$\\[1.0ex]
$0.001$&$1.1179$&$3.9007\rme-1$&$1.5080$&$1.5186$&$1.525$\\[1.0ex]
$0.0001$&$1.4843$&$1.1301$&$2.6144$&$2.7104$&$2.712$\\[1.0ex]
\hline
\end{tabular}
\caption{\footnotesize $G(r)$ the exact 2-point function, 
and $G_1(r),G_3(r)$ the 1-- and 3--particle contributions.} 
\label{Ising2pt}
\end{table}

In table \ref{Ising2pt} various contributions are given.
The full function is solved by integrating from $x=10^{-4}$ in wf\_solve\_phi.f
using a NAGLIB routine (the results agree with Janos) and the 3--particle
contribution is programmed in wf\_g3.f.
We see that $G_1(r)+G_3(r)$ is a good approximation right down to $r=0.01$
and even at $r=0.001$ there is only a $\sim1\%$ error.


\subsection{2--particle wave functions}

Define two-particle wave functions by
\be
\Psi(r,\theta)=
i\langle 0|\sigma((0,x_1))\sigma(0)|\theta,-\theta\rangle^{\rm in}\,,
\end{equation}
where $\theta\ge0$; the fields are at equal time (and $x_1$ 
is the spatial coordinate) and
\be
r\equiv Mx_1\,.
\end{equation}
Parity invariance (and locality) implies
\be
\Psi(r,\theta)=\Psi(-r,\theta)\,.
\end{equation}
Using completeness we $\Psi$ can be expressed as a sum over $s$-particle
contributions
\be
\Psi(r,\theta)=\sum_{s=1}^{\infty}\Psi_{2s-1}(r,\theta)\,.
\end{equation}

\subsubsection{1--particle contribution}

For the 1--particle contribution we have
\be
\Psi_1(r,\theta)=c_1 T(2\theta) p_1(r,\theta)\,,
\end{equation}
with
\be
c_1=i\frac{2i}{4\pi}=-\frac{1}{2\pi}\,,
\end{equation}
and
\be
p_1(r,\theta)=\int_{-\infty}^\infty\rmd\theta_1\,\rme^{i|r|\sh\theta_1}
\frac{{\cal P}}{T(\theta_1-\theta)T(\theta_1+\theta)}\,.
\end{equation}
Now use
\be
\frac{\cal P}{T(\phi)}=2\pi i\delta(\phi)+\frac{1}{T(\phi+i\epsilon)}\,,
\end{equation}
to obtain
\be
p_1=p_1^{(2)}+p_1^{(1)}+p_1^{(0)}\,,
\end{equation}
where the superscripts denote the number of delta functions. So
\ba
p_1^{(2)}(r,\theta)&=&(2\pi i)^2
\int_{-\infty}^{\infty}\rmd\theta_1\,\rme^{i|r|\sh\theta_1}
\delta(\theta_1-\theta)\delta(\theta_1+\theta)
\\
&=&-2\pi^2\delta(\theta)\,.
\ea
Next
\ba
p_1^{(1)}(r,\theta)&=&2\pi i
\int_{-\infty}^{\infty}\rmd\theta_1\,\rme^{i|r|\sh\theta_1}
\left[\frac{\delta(\theta_1-\theta)}{T(\theta_1+\theta+i\epsilon)}
     +\frac{\delta(\theta_1+\theta)}{T(\theta_1-\theta+i\epsilon)}\right]
\nonumber\\
&&
\\
&=&2\pi i\left[\frac{\rme^{ i|r|\sh\theta}}{T(2\theta+i\epsilon)}
              -\frac{\rme^{-i|r|\sh\theta}}{T(2\theta-i\epsilon)}
\right]
\\
&=&4\pi^2\delta(\theta)-4\pi\frac{\sin(|w|\sh\theta)}{T(2\theta)}\,.
\ea
Finally
\be
p_1^{(0)}(r,\theta)=\int_{-\infty}^\infty 
\rmd\theta_1\,\rme^{i|r|\sh\theta_1}
\frac{1}{T(\theta_1-\theta+i\epsilon)T(\theta_1+\theta+i\epsilon)}\,.
\end{equation}
Shifting the contour to the line parallel to the real axis with
imaginary part $i\pi/2$ (and observing that the contribution from the 
contours parallel to the imaginary axis at infinity is zero for 
$r\ne 0$) we get
\ba
p_1^{(0)}(r,\theta)&=&-\int_{-\infty}^\infty\rmd z\,
\rme^{-|r|\ch z}\frac{\ch\theta+i\sh z}{\ch\theta-i\sh z}
\\
&=&2K_0(|r|)-4\ch^2\theta\int_0^\infty\rmd z\,
\frac{\rme^{-|r|\ch z}}{\ch^2\theta+\sh^2 z}\,.
\ea
Summarizing we have
\be
\Psi_1(r,\theta)=-c_1\left[4\pi\sin(|r|\sh\theta)
-T(2\theta)p_1^{(0)}(r,\theta)\right]\,.
\end{equation}
The plane wave part is as expected for a two particle S-matrix
equal to $-1$; and $p_1^{(0)}(r,\theta)$ decays exponentially
as $|r|\to\infty$.

\subsubsection{3--particle contribution}

For the 3--particle contribution we have
\be
\Psi_3(r,\theta)=c_3 T(2\theta) p_3(r,\theta)\,,
\end{equation}
with
\be
c_3=i\frac{(-2i)(2i)^2}{(4\pi)^3}=-\frac{1}{8\pi^3}\,,
\end{equation}
and
\ba
p_3(r,\theta)&=&\int_0^\infty\rmd u_1\,\rmd u_2\int_{-\infty}^\infty
\rmd\Lambda\,\rme^{i|r|\mu^{(3)}(u)\sh\Lambda}
\left[T(u_1)T(u_2)T(u_1+u_2)\right]^2
\nonumber\\
&&\times\prod_{j=1}^3
\frac{{\cal P}}{T(\theta_j-\theta)T(\theta_j+\theta)}\,,
\ea
and
\be
\mu^{(3)}(u)=\sqrt{3+2\ch u_1+2\ch u_2+2\ch u_{12}}\,.
\end{equation}
In the decomposition of the principle parts we have
(ignoring terms involving $\delta(\theta)$) 
\be
p_3=p_3^{(2)}+p_3^{(1)}+p_3^{(0)}
\end{equation}
because the term involving three delta functions involving the
different $\theta_j$ would require $u_1=0$ and/or $u_2=0$
and its contribution vanishes because of the $T(u_1)T(u_2)$ factors
in the integrand. 
We get (for $\theta>0$):
\ba 
&&p_3^{(2)}(r,\theta)=-(2\pi i)^2\frac{1}{T(2\theta)^2}
\int_0^\infty\rmd u_1\,\rmd u_2\int_{-\infty}^\infty
\rmd\Lambda\,\rme^{i|r|\mu^{(3)}(u)\sh\Lambda}
\left[T(u_1)T(u_2)T(u_{12})\right]^2
\nonumber\\
&&\times\Bigl[\delta(u_{13}+\Lambda-\theta)\delta(u_{23}+\Lambda+\theta)
\frac{1}{T(u_3+\Lambda-\theta+i\epsilon)T(u_3+\Lambda+\theta+i\epsilon)}
\nonumber\\
&&+\delta(u_{13}+\Lambda-\theta)\delta(u_3+\Lambda+\theta)
\frac{1}{T(u_{23}+\Lambda-\theta+i\epsilon)T(u_{23}+\Lambda+\theta+i\epsilon)}
\nonumber\\
&&+\delta(u_{23}+\Lambda-\theta)\delta(u_3+\Lambda+\theta)
\frac{1}{T(u_{13}+\Lambda-\theta+i\epsilon)
T(u_{13}+\Lambda+\theta+i\epsilon)}\Bigr]
\nonumber\\
&&
\\
&=&4\pi^2\int_0^\infty\rmd u_2\,
\rme^{-i|r|\sh(u_2+\theta)}T(u_2)T(2\theta+u_2)
\nonumber\\
&&-4\pi^2\int_0^{2\theta}\rmd u_2\,
\rme^{i|r|\sh(u_2-\theta)}T(2\theta-u_2)T(u_2)
\nonumber\\
&&+4\pi^2\int_0^\infty\rmd u_1\,
\rme^{i|r|\sh(u_1+\theta)}T(u_1)T(u_1+2\theta)
\\
&&
\nonumber\\
&=&8\pi^2\int_0^\infty\rmd v\,
\cos(|r|\sh v)T(v+\theta)T(v-\theta)
\\
&=&8\pi^2\left[K_0(|r|)-2\ch\theta\int_0^\infty\rmd v\,
\frac{\cos(|r|\sh v)}{\ch v+\ch\theta}\right]
\\
&=&4\pi^2 p_1^{(0)}(r,\theta)\,,
\ea
where we have used Eq.~(\ref{besselK0}).

Next 
\ba 
p_3^{(1)}(r,\theta)&=&\frac{2\pi i}{T(2\theta)}
\int_0^\infty\rmd u_1\,\rmd u_2\, T(u_1)T(u_2)T(u_{12}) 
\nonumber\\
&&\times\Bigl\{\Bigl[
\frac{T(u_2)\rme^{i|r|\mu^{(3)}(u)\sh(\theta-u_{13})}}
{T(u_1-2\theta-i\epsilon)T(u_{12}-2\theta-i\epsilon)} 
\nonumber\\
&&+\frac{T(u_{12})\rme^{i|r|\mu^{(3)}(u)\sh(\theta-u_{23})}}
{T(u_2-2\theta-i\epsilon)T(u_1+2\theta+i\epsilon)} 
\nonumber\\
&&+\frac{T(u_1)\rme^{i|r|\mu^{(3)}(u)\sh(\theta-u_3)}}
{T(u_2+2\theta+i\epsilon)T(u_{12}+2\theta+i\epsilon)}\Bigr] 
\nonumber\\
&&-\Bigl[{\rm all\,\,terms}\,\,\theta\to-\theta\Bigr]\Bigr\}\,. 
\ea
Finally 
\ba 
&&p_3^{(0)}(r,\theta)=-\int_0^\infty\rmd u_1\,\rmd u_2\,
\int_{-\infty}^\infty \rmd z\,\rme^{-|r|\mu^{(3)}(u)\ch z}
\left[T(u_1)T(u_2)T(u_{12})\right]^2 
\nonumber\\ 
&&\times\left\{
\frac{[\ch\theta+i\sh(u_{13}+z)][\ch\theta+i\sh(u_{23}+z)]
 [\ch\theta+i\sh(u_3+z)]}
     {[\ch\theta-i\sh(u_{13}+z)][\ch\theta-i\sh(u_{23}+z)]
 [\ch\theta-i\sh(u_3+z)]}\right\}\,.
\nonumber\\
&&
\ea

Noting 
\ba
\mu^{(3)}(u)\sh u_3&=&-\sh u_2 -\sh u_{12}\,,
\\
\mu^{(3)}(u)\ch u_3&=&1+\ch u_2 +\ch u_{12}\,,
\ea
we have
\ba 
&&p_3^{(0)}(r,\theta)=-2{\rm Re}\int_0^\infty\rmd u_1\,\rmd u_2\,
\int_0^\infty \rmd z\,\rme^{-|r|\mu^{(3)}(u)\ch z}
\left[T(u_1)T(u_2)T(u_{12})\right]^2 
\nonumber\\ 
&&\times Z(u,z,\theta;u_1,u_{12})
Z(u,z,\theta;-u_1,u_2)Z(u,z,\theta;-u_2,-u_{12})\,,
\nonumber\\
&&
\ea
where
\be
Z(u,\theta;z,a,b)=\frac{\mu^{(3)}(u)\ch\theta+i[\sh z+\sh(z+a)+\sh(z+b)]}
                       {\mu^{(3)}(u)\ch\theta-i[\sh z+\sh(z+a)+\sh(z+b)]}\,.
\end{equation}
Also
\ba 
p_3^{(1)}(r,\theta)&=&\frac{2\pi i}{T(2\theta)}
\int_0^\infty\rmd u_1\,\rmd u_2\, T(u_1)T(u_2)T(u_{12}) 
\nonumber\\
&&\times\Bigl\{\rme^{i|r|\sh\theta} \Bigl[
   \frac{T(u_2)   \rme^{i|r|\{\sh(\theta-u_1)+\sh(\theta-u_{12})\}}}
{T(u_1-2\theta-i\epsilon)T(u_{12}-2\theta-i\epsilon)} 
\nonumber\\
&&+\frac{T(u_{12})\rme^{i|r|\{\sh(\theta-u_2)+\sh(\theta+u_1)   \}}}
{T(u_2-2\theta-i\epsilon)T(u_1+2\theta+i\epsilon)} 
\nonumber\\
&&+\frac{T(u_1)   \rme^{i|r|\{\sh(\theta+u_2)+\sh(\theta+u_{12})\}}}
{T(u_2+2\theta+i\epsilon)T(u_{12}+2\theta+i\epsilon)}\Bigr] 
\nonumber\\
&&-\Bigl[{\rm all\,\,terms}\,\,\theta\to-\theta\Bigr]\Bigr\}\,. 
\ea

Distorting the contours we get
\be 
p_3^{(1)}(r,\theta)=\frac{2\pi i}{T(2\theta)}
\sum_{s=1}^8\left[\rme^{i|r|\sh\theta}A_s(r,\theta)
-(\theta\rightarrow -\theta)\right]\,,
\end{equation}
with
\ba
A_1(r,\theta)
&=&-i\int_0^{\pi/2}\rmd z\,\int_0^\infty\rmd u_2\, T(-iz)T(u_2)T(-iz+u_2) 
\nonumber\\
&&\times\frac{T(u_2)   
\rme^{i|r|\{\cos z[\sh\theta+\sh(\theta-u_2)]
               +i\sin z[\ch\theta+\ch(\theta-u_2)]\}}}
{T(-iz-2\theta)T(-iz+u_2-2\theta)}\,, 
\\
A_2(r,\theta)&=&\int_0^\infty\rmd z\int_0^\infty\rmd u_2\, 
T(z-i\pi/2)T(u_2)T(z-i\pi/2+u_2) 
\nonumber\\
&&\times\frac{T(u_2)\rme^{-|r|\{\ch(\theta-z)+\ch(\theta-u_2-z)\}}}
{T(z-i\pi/2-2\theta)T(z-i\pi/2+u_2-2\theta)}\,, 
\\
A_3(r,\theta)&=&
\int_0^{\pi/2}\rmd w\int_0^{\pi/2}\rmd z\, T(iw)T(-iz)T(i(w-z)) 
\nonumber\\
&&\times\frac{T(i(w-z))\rme^{i|r|\{\sh(\theta+iz)+\sh(\theta+iw)\}}}
{T(-iz-2\theta)T(iw+2\theta)}\,, 
\\
A_4(r,\theta)&=&-i\int_0^\infty\rmd w\,\,\int_0^{\pi/2}\rmd z\, 
T(w+i\pi/2)T(w-iz+i\pi/2)T(-iz) 
\nonumber\\
&&\times\frac{T(w-iz+i\pi/2)\rme^{i|r|\{\sh(\theta+iz)+i\ch(\theta+w)\}}}
{T(-iz-2\theta)T(w+i\pi/2+2\theta)}\,, 
\\
A_5(r,\theta)&=&i\int_0^\infty\rmd z\,\int_0^{\pi/2}\rmd w\, 
T(iw)T(z-i\pi/2)T(z+iw-i\pi/2) 
\nonumber\\
&&\times\frac{T(z+iw-i\pi/2)   
\rme^{i|r|\{i\ch(\theta-z)+\sh(\theta+iw)\}}}
{T(z-i\pi/2-2\theta)T(iw+2\theta)}\,, 
\\
A_6(r,\theta)&=&\int_0^\infty\rmd w\,\int_0^\infty\rmd z\, 
T(w+i\pi/2)T(z-i\pi/2)T(w+z) 
\nonumber\\
&&\times\frac{T(w+z)\rme^{-|r|\{\ch(\theta-z)+\ch(\theta+w)\}}}
{T(z-i\pi/2-2\theta)T(w+i\pi/2+2\theta)}\,, 
\\
A_7(r,\theta)&=&i\int_0^\infty\rmd u_1\,\int_0^{\pi/2}\rmd z\, 
T(u_1)T(iz)T(u_1+iz) 
\nonumber\\
&&\times\frac{T(u_1)\rme^{i|r|\{\cos z[\sh\theta+\sh(\theta+u_1)]
                                   +i\sin z[\ch\theta+\ch(\theta+u_1)]\}}}
{T(iz+2\theta)T(iz+u_1+2\theta)}\,, 
\\
A_8(r,\theta)&=&\int_0^\infty\rmd u_1\,\int_0^\infty\rmd z\, 
T(u_1)T(z+i\pi/2)T(u_1+z+i\pi/2) 
\nonumber\\
&&\times\frac{T(u_1)\rme^{-|r|\{\ch(\theta+z)+\ch(\theta+z+u_1)\}}}
{T(z+i\pi/2+2\theta)T(z+i\pi/2+u_1+2\theta)}\,. 
\ea
Note
\ba
A_3(r,\theta)&=&A_3(r,-\theta)^*\,,
\\
A_6(r,\theta)&=&A_6(r,-\theta)^*\,,
\\
A_5(r,\theta)&=&A_4(r,-\theta)^*\,,
\\
A_7(r,\theta)&=&A_1(r,-\theta)^*\,,
\\
A_8(r,\theta)&=&A_2(r,-\theta)^*\,.
\ea
So we have
\ba
p_3^{(1)}(r,\theta)&=&\frac{-4\pi}{T(2\theta)}\sum_{s=1,2,3,4,6}c_s
\nonumber\\
&&\times\Bigl\{\sin(|r|\sh\theta){\rm Re}
[A_s(r,\theta)+A_s(r,-\theta)] 
\nonumber\\
&&+\cos(|r|\sh\theta){\rm Im}
[A_s(r,\theta)-A_s(r,-\theta)]\Bigr\}\,,
\ea
with $c_1=c_2=c_4=1\,,c_3=c_6=1/2$.

\begin{table}[h]
\centering
\begin{tabular}[t]{l|l|l|l}
\hline
$r$&
$p_3^{(2)}(r,0.1)\quad\,\,\,$&
$p_3^{(1)}(r,0.1)\quad\,\,\,$&  
$p_3^{(0)}(r,0.1)$\\[1.0ex]
\hline \hline
$10.0$&$-1.177627154\rme-3$&$-7.69650\rme-7$&$-5.5\rme-19$\\[1.0ex]
$5.0$&$-2.110316\rme-1$&$-1.88350\rme-4$&$-2.0\rme-11$\\[1.0ex]
$4.0$&$-5.967461\rme-1$&$-1.9768\rme-3$&$-8.3\rme-10$\\[1.0ex]
$3.0$&$-1.673215$&$-2.06642\rme-2$&$-4.0\rme-8$\\[1.0ex]
$2.0$&$-4.531142$&$-2.43433\rme-1$&$-2.5\rme-6$\\[1.0ex]
$1.0$&$-1.006191\rme+1$&$-3.75516$&$-2.47622\rme-4$\\[1.0ex]
$0.1$&$\phantom{-}5.500439\rme+1$&$-1.37409\rme+2$&$\phantom{-}6.39684\rme-2$\\[1.0ex]
$0.01$&$\phantom{-}2.167782\rme+2$&$-4.41605\rme+2$&$\phantom{-}8.03367$\\[1.0ex]
$0.001$&$\phantom{-}3.963772\rme+2$&$-7.94359\rme+2$&$\phantom{-}6.79629\rme+1$\\[1.0ex]
\hline
\end{tabular}
\caption{\footnotesize Contributions to the 3--particle 
contribution to the wave function for $\theta=0.1$.} 
\label{Psi3t01}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}[t]{l|l|l|l}
\hline
$r$ &
$p_3^{(2)}(r,0.3)\quad\,\,\,$&
$p_3^{(1)}(r,0.3)\quad\,\,\,$&  
$p_3^{(0)}(r,0.3)$\\[1.0ex]
\hline \hline
$10.0$&$-1.191534\rme-3$&$\phantom{-}1.60099\rme-7$&$-5.6\rme-19$\\[1.0ex]
$5.0$&$-2.153397\rme-1$&$-5.09090\rme-5$&$-2.1\rme-11$\\[1.0ex]
$4.0$&$-6.111677\rme-1$&$-7.89360\rme-4$&$-8.6\rme-10$\\[1.0ex]
$3.0$&$-1.723368$&$-1.13509\rme-2$&$-4.1\rme-8$\\[1.0ex]
$2.0$&$-4.715949$&$-1.71485\rme-1$&$-2.5\rme-6$\\[1.0ex]
$1.0$&$-1.081669\rme+1$&$-3.12477$&$-2.58618\rme-4$\\[1.0ex]
$0.1$&$\phantom{-}5.162984\rme+1$&$-1.31757\rme+2$&$\phantom{-}4.14019\rme-2$\\[1.0ex]
$0.01$&$\phantom{-}2.126917\rme+2$&$-4.33754\rme+2$&$\phantom{-}7.50810$\\[1.0ex]
$0.001$&$\phantom{-}3.922039\rme+2$&$-7.86077\rme+2$&$\phantom{-}6.54232\rme+1$\\[1.0ex]
\hline
\end{tabular}
\caption{\footnotesize Contributions to the 3--particle 
contribution to the wave function for $\theta=0.3$.} 
\label{Psi3t03}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}[t]{l|l|l|l}
\hline
$r$ &
$p_3^{(2)}(r,1.0)\quad\,\,\,$&
$p_3^{(1)}(r,1.0)\quad\,\,\,$&  
$p_3^{(0)}(r,1.0)$\\[1.0ex]
\hline \hline
$10.0$&$-1.294659\rme-3$&$-2.99547\rme-11$&$-6.7\rme-19$\\[1.0ex]          
$5.0$&$-2.493382\rme-1$&$-1.27569\rme-5$&$-2.7\rme-11$\\[1.0ex]
$4.0$&$-7.275435\rme-1$&$-3.74861\rme-4$&$-1.1\rme-9$\\[1.0ex]
$3.0$&$-2.140146$&$-1.22519\rme-3$&$-5.6\rme-8$\\[1.0ex]
$2.0$&$-6.316308$&$\phantom{-}5.31559\rme-2$&$-3.6\rme-6$\\[1.0ex]
$1.0$&$-1.778817\rme+1$&$\phantom{-}7.79587\rme-1$&$-3.76813\rme-4$\\[1.0ex]
$0.1$&$\phantom{-}1.654539\rme+1$&$-7.51139\rme+1$&$-1.30180\rme-1$\\[1.0ex]
$0.01$&$\phantom{-}1.691532\rme+2$&$-3.50663\rme+2$&$\phantom{-}2.81568$\\[1.0ex]
$0.001$&$\phantom{-}3.476033\rme+2$&$-6.97670\rme+2$&$\phantom{-}4.08945\rme+1$\\[1.0ex]
\hline
\end{tabular}
\caption{\footnotesize Contributions to the 3--particle 
contribution to the wave function for $\theta=1.0$.} 
\label{Psi3t10}
\end{table}


\subsubsection{Exact result from Fronseca and Zamolodchikov}

Let $\widetilde{\Psi}(r,\theta)$ be the corresponding wave function 
for the disorder variables
\be
\widetilde{\Psi}(r,\theta)=
i\langle 0|\mu((0,x_1))\mu(0)|\theta,-\theta\rangle^{\rm in}\,,
\end{equation}
and define
\be
\Psi_\pm=\widetilde{\Psi}\pm\Psi\,.
\end{equation}
Then Fronseca and Zamolodchikov claim that the exact result is given by
\be
\Psi_\pm(r,\theta)=\frac{G_\pm(r)}{\ch\theta}\left[
\rme^{-\theta}\Phi_\pm(r,\theta)^2-\rme^{\theta}\Phi_\mp(r,\theta)^2\right]\,,
\end{equation}
where $G_\pm$ are defined through the vacuum two-point 
functions in (\ref{Gplusminus}) and $\Phi_\pm$ are the functions 
$\Psi_\pm$ in the notation of Fronseca and Zamolodchikov 
(and we have used the relation $\Phi_\pm(r,\theta)=\Phi_\mp(r,-\theta)$), 
which satisfy the coupled equations
\be
\Phi'_\pm(r,\theta)=\frac12\sh(\varphi(r)\pm\theta)\Phi_\mp(r,\theta)\,.
\end{equation}
For small $r$ we have
\be
\rme^{\chi(r)/2}\Phi_\pm(r,\theta)\sim\sqrt{2\pi}C_\chi\rme^{\pm\theta/2}
r^{1/4}\left[1+\rmO(r^2)\right]\,.
\end{equation}

The wave function $\Psi$ is then given by
\be
\Psi(r,\theta)=\frac{\rme^{\chi(r)/2}}{\ch\theta}\left[
 \Phi_+(r,\theta)^2\cosh\left(\frac{\varphi(r)}{2}-\theta\right)
-\Phi_-(r,\theta)^2\cosh\left(\frac{\varphi(r)}{2}+\theta\right)\right]\,.
\end{equation}
For small $r$ it has the expansion
\be
\Psi(r,\theta)\sim 2\pi C_\chi r^{3/4}\sinh\theta+\dots\,.
\end{equation}


Expanding $\Phi_\pm(r,\theta)$ for small $\theta$
\be
\Phi_\pm(r,\theta)=\Phi_0(r)\pm\theta\Phi_1(r)+\dots
\end{equation}
and defining
\ba
\mu(r)&=&\Phi_0(r)^2\,,
\\
\nu(r)&=&2\Phi_0(r)\Phi_1(r)\,,
\ea
we have
\ba
\mu'(r)&=&\mu(r)\sinh\varphi(r)\,,
\\
\nu'(r)&=&\mu(r)\cosh\varphi(r)\,.
\ea
Then for small $\theta$ we have
\be
\Psi(r,\theta)\sim 2\theta\rme^{\chi(r)/2}
\left[\nu(r)\cosh\frac{\varphi(r)}{2}
-\mu(r)\sinh\frac{\varphi(r)}{2}\right]+\dots
\end{equation}
and 
\ba
&&V_0(r):=\lim_{\theta\to0}\frac{\Psi''(r,\theta)}{\Psi(r,\theta)}
\\
&&=\frac14\left[\chi'(r)\left(\frac{2}{r}+\chi'(r)\right)-\varphi'(r)^2\right]
\nonumber\\
&&+\frac{\left[\{\chi'(r)\varphi'(r)+\varphi''(r)\}
\{\nu(r)\sinh\frac{\varphi(r)}{2}-\mu(r)\cosh\frac{\varphi(r)}{2}\}
+2\mu(r)\{\chi'(r)+\sinh\varphi(r)\}\cosh\frac{\varphi(r)}{2}\right]}
{2\left[\nu(r)\cosh\frac{\varphi(r)}{2}-\mu(r)\sinh\frac{\varphi(r)}{2}\right]}\,.
\nonumber\\
&&
\ea

\begin{table}[h]
\centering
\begin{tabular}[t]{l|l|l|l|l|l}
\hline
$r$ &
$\Psi_1(r,0.1)$\quad\,\,\,&
$\Psi_3(r,0.1)$\quad\,\,\,&  
$[\Psi_1+\Psi_3](r,0.1)$\quad\,\,\,&  
$\Psi(r,0.1)$\quad\,\,\,&  
$\Psi_{\rm as}(r,0.1)$\\[1.0ex]
\hline \hline
$10.0$&$\phantom{-}1.68474$&$4.73487\rme-7$&$\phantom{-}1.68474$&$1.68474$&\\[1.0ex]
$5.0$&$\phantom{-}9.60399\rme-1$&$8.48694\rme-5$&$\phantom{-}9.60484\rme-1$&$9.60484\rme-1$&\\[1.0ex]
$4.0$&$\phantom{-}7.80305\rme-1$&$2.40570\rme-4$&$\phantom{-}7.80546\rme-1$&$7.80546\rme-1$&\\[1.0ex]
$3.0$&$\phantom{-}5.92668\rme-1$&$6.80610\rme-4$&$\phantom{-}5.93349\rme-1$&$5.93349\rme-1$&\\[1.0ex]
$2.0$&$\phantom{-}3.99813\rme-1$&$1.91841\rme-3$&$\phantom{-}4.01731\rme-1$&$4.01731\rme-1$&\\[1.0ex]
$1.0$&$\phantom{-}2.04042\rme-1$&$5.55188\rme-2$&$\phantom{-}2.09594\rme-1$&$2.09594\rme-1$&\\[1.0ex]
$0.1$&$-2.06806\rme-3$&$3.30849\rme-2$&$\phantom{-}3.10168\rme-2$&$3.11080\rme-2$&$3.03513\rme-2$\\[1.0ex]
$0.01$&$-8.50994\rme-2$&$8.71087\rme-2$&$\phantom{-}2.0093\rme-3$&$5.41080\rme-3$&$5.39731\rme-3$\\[1.0ex]
$0.001$&$-1.59066$&$1.32604\rme-1$&$-1.458056$&$9.60032\rme-4$&$9.59792\rme-4$\\[1.0ex]
$0.0001$&$ $&$ $&$ $&$1.70682\rme-4$&$1.70678\rme-4$\\[1.0ex]
\hline
\end{tabular}
\caption{\footnotesize $\Psi(r,\theta)$ the exact wave function function, 
and $\Psi_1(r,\theta),\Psi_3(r,\theta)$ the 1-- and 3--particle 
contributions for $\theta=0.1$.} 
\label{Isingwavefn01}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}[t]{l|l|l|l|l|l}
\hline
$r$ &
$\Psi_1(r,0.3)$\quad\,\,\,&
$\Psi_3(r,0.3)$\quad\,\,\,&  
$[\Psi_1+\Psi_3](r,0.3)$\quad\,\,\,&  
$\Psi(r,0.3)$\quad\,\,\,&  
$\Psi_{\rm as}(r,0.3)$\\[1.0ex]
\hline \hline
$10.0$&$\phantom{-}1.92482\rme-1$&$1.39916\rme-6$&$\phantom{-}1.92484\rme-1$&$1.92484\rme-1$&\\[1.0ex]
$5.0$&$\phantom{-}1.99793$&$2.52957\rme-4$&$\phantom{-}1.99818$&$1.99818$&\\[1.0ex]
$4.0$&$\phantom{-}1.87759$&$7.18688\rme-4$&$\phantom{-}1.87831$&$1.87831$&\\[1.0ex]
$3.0$&$\phantom{-}1.58539$&$2.03727\rme-3$&$\phantom{-}1.58743$&$1.58743$&\\[1.0ex]
$2.0$&$\phantom{-}1.14970$&$5.73985\rme-3$&$\phantom{-}1.15544$&$1.15544$&\\[1.0ex]
$1.0$&$\phantom{-}6.12374\rme-1$&$1.63733\rme-2$&$\phantom{-}6.28747$&$6.28748\rme-1$&\\[1.0ex]
$0.1$&$\phantom{-}2.60053\rme-4$&$9.40535\rme-2$&$\phantom{-}9.43136\rme-2$&$9.45618\rme-2$&$9.22720\rme-2$\\[1.0ex]
$0.01$&$-2.43697\rme-1$&$2.50800\rme-1$&$\phantom{-}7.10370\rme-3$&$1.64495\rme-2$&$1.64085\rme-2$\\[1.0ex]
$0.001$&$-4.59999\rme-1$&$3.85735\rme-1$&$-7.42642\rme-2$&$2.91863\rme-3$&$2.91790\rme-3$\\[1.0ex]
$0.0001$&$ $&$ $&$ $&$5.18897\rme-4$&$5.18884\rme-4$\\[1.0ex]
\hline
\end{tabular}
\caption{\footnotesize As in Table~\ref{Isingwavefn01} but here for 
$\theta=0.3$.} 
\label{Isingwavefn03}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}[t]{l|l|l|l|l|l}
\hline
$r$ &
$\Psi_1(r,1.0)$\quad\,\,\,&
$\Psi_3(r,1.0)$\quad\,\,\,&  
$[\Psi_1+\Psi_3](r,1.0)$\quad\,\,\,&  
$\Psi(r,1.0)$\quad\,\,\,&  
$\Psi_{\rm as}(r,1.0)$\\[1.0ex]
\hline \hline
$10.0$&$-1.45457$&$3.97502\rme-6$&$-1.45457$&$-1.45456$&\\[1.0ex]
$5.0$&$-7.91276\rme-1$&$7.65588\rme-4$&$-7.90510\rme-1$&$-7.90511\rme-1$&\\[1.0ex]
$4.0$&$-1.99763$&$2.23494\rme-3$&$-1.99540$&$-1.99540$&\\[1.0ex]
$3.0$&$-7.42714\rme-1$&$6.57470\rme-3$&$-7.36139\rme-1$&$-7.36139\rme-1$&\\[1.0ex]
$2.0$&$\phantom{-}1.44177$&$1.92299\rme-2$&$\phantom{-}1.46100$&$\phantom{-}1.46100$&\\[1.0ex]
$1.0$&$\phantom{-}1.90015$&$5.22230\rme-2$&$\phantom{-}1.95237$&$\phantom{-}1.95237$&\\[1.0ex]
$0.1$&$\phantom{-}1.83700\rme-1$&$1.80224\rme-1$&$\phantom{-}3.63924\rme-1$&$\phantom{-}3.64293\rme-1$&$3.56095\rme-1$\\[1.0ex]
$0.01$&$-4.95851\rme-1$&$5.48649\rme-1$&$\phantom{-}5.2798\rme-2$&$\phantom{-}6.34808\rme-2$&$6.33237\rme-2$\\[1.0ex]
$0.001$&$-1.06490$&$9.49258\rme-1$&$-1.15642\rme-1$&$\phantom{-}1.12635\rme-2$&$1.12607\rme-2$\\[1.0ex]
$0.0001$&$ $&$ $&$ $&$\phantom{-}2.00252\rme-3 $&$2.00247\rme-3$\\[1.0ex]
\hline
\end{tabular}
\caption{\footnotesize As in Table~\ref{Isingwavefn01} but here for 
$\theta=1.0$.} 
\label{Isingwavefn1.0}
\end{table}



\vfill
\eject







                            


         

